An Agent-based Model of Contagion in Financial Networks

This work develops an agent-based model for the study of how the leverage through the use of repurchase agreements can function as a mechanism for the propagation and amplification of financial shocks in a financial system. Based on the analysis of financial intermediaries in the repo and interbank lending markets during the 2007-08 financial crisis we develop a model that can be used to simulate the dynamics of financial contagion.

==> placeholder.tex <==
The model: SIS spread of risk}
Another way to look at the spread of risk in the network of financial firms as described above, is to model it as an epidemic process. Here we will adopt the individual-based mean-field approach, described by \citet{Pastor-Satorras_Castellano_Van_Mieghem_Vespignani_2015}, to model spread of risk as an SIS model (Susceptible-Infected-Susceptible).

We start by defining the \emph{infected} state ($I$) as the status where  it's value has dropped below a certain value. We also assume, as in the previous model, that if a fund is in the $I$ state, it can also "infect" others, i.e., increase the probability of its neighbors to also make the transition to the $I$ state.

Given a network topology described by an adjacency matrix $a_{ij}$, the probability of an organization $i$ being infected is given by:
\begin{align}\label{eq:sis1}
\frac{d\rho_i^I(t)}{dt}= -\mu \rho_i^I(t) +\beta [1-\rho_i^I(t)]\sum_{j=1}^N a_{ij}\rho_i^I(t)
\end{align}

Without loss of generality we can rescale $t$ by $1/\mu$, so the recovery rate, $\mu$ is unitary.  If we also make $\lambda=\beta/\mu$. we get an adimensional effective transmission rate, and equation \ref{eq:sis1}  becomes
\begin{align}\label{eq:sis2}
\frac{d\rho_i^I(t)}{dt}= -\rho_i^I(t) +\lambda [1-\rho_i^I(t)]\sum_{j=1}^N a_{ij}\rho_i^I(t)
\end{align}
See eq. 33 in \citet{Pastor-Satorras_Castellano_Van_Mieghem_Vespignani_2015} for a derivation of the above equations. 

In our network of funds, we have weighted connections between organizations. In order to take this into account we can simply replace the adjacency matrix $a_{ij}$ by $\Omega_{ij}= \omega_{ij}a_{ij}$. By doing this, we are saying that the rate of transmission between two adjacent nodes is a function of their weight of the edge  connecting them.
